A Computationally Efficient Neural Network Invariant to the Action of Symmetry Subgroups

We introduce a method to design a computationally efficient $G$-invariant neural network that approximates functions invariant to the action of a given permutation subgroup $G \leq S_n$ of the symmetric group on input data. The key element of the proposed network architecture is a new $G$-invariant transformation module, which produces a $G$-invariant latent representation of the input data. This latent representation is then processed with a multi-layer perceptron in the network. We prove the universality of the proposed architecture, discuss its properties and highlight its computational and memory efficiency. Theoretical considerations are supported by numerical experiments involving different network configurations, which demonstrate the effectiveness and strong generalization properties of the proposed method in comparison to other $G$-invariant neural networks.

==> abandoned.tex <==
% \section{Example}
% For example: Let $x = (a, b, c, d) \in \mathbb{R}^{4 \times 2}$, $G = (1324)$
% \begin{equation}
% \begin{split}
%     &f_{in}(x) = f_{in}(a, b, c, d) = \\
%     & \begin{bmatrix} 
%     \phi_1(a) & \phi_2(a) & \phi_3(a) & \phi_4(a)\\
%     \phi_1(b) & \phi_2(b) & \phi_3(b) & \phi_4(b)\\
%     \phi_1(c) & \phi_2(c) & \phi_3(c) & \phi_4(c)\\
%     \phi_1(d) & \phi_2(d) & \phi_3(d) & \phi_4(d)\\
%     \end{bmatrix} \in \mathbb{R}^{4 \times 4 \times 64}\\
% \end{split},
% \end{equation}
% where $\phi_1, \phi_2, \phi_3, \phi_4$ are nonlinear, pairwise linearly independent functions. Then
% \begin{equation}
% \begin{split}
%     \Sigma\Pi(f_{in}(a, b, c, d)) & = \phi_1(a)\phi_2(b)\phi_3(c)\phi_4(d) \\
%     & + \phi_3(a)\phi_2(b)\phi_4(c)\phi_1(d) \\
%     & + \phi_2(a)\phi_4(b)\phi_1(c)\phi_3(d) \\
%     & + \phi_4(a)\phi_1(b)\phi_3(c)\phi_2(d) \in \mathbb{R}^{n_{mid}}\\
% \end{split},
% \end{equation}
% which can be considered as the $G$-invariant feature vector of the input. Finally, that representation is transformed by the $f_{out}$ function, which can be approximated by the neural network.




% For outdated version of n-gon estimation
% The goal of this experiment is to asses how the performance of the different $G$-invariant models changes with the increasing size of the input and the group. To evaluate that, convex $n$-gon area estimation task was realized (in the same setup as for convex quadrangle area estimation) and results on the test dataset are reported in Table \ref{tab:ngons}.

% Obtained results show that for all tested $n$-gons Conv1D $G$-inv model outperforms other tested approaches.
% One can see, that for almost all models MAE increases with the growth of $n$. That behavior is also obtained for the proposed $G$-invariant architecture, which agrees with the theoretical considerations, that the upper bound of the error grows with the growth of $n$ and $m$. Although the upper bound grows with $mn$, fortunately the obtained MAE does not grow so fast.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% NGONs
% \begin{table*}[t]
% \caption{Mean absolute errors [$10^{-3} \text{unit}^2$] and mean running times [ms] in the task of convex n-gon area estimation for several $G$-invariant models. Presented numbers are the mean and standard deviation of MAE for 10 different model instances.}
% \label{tab:ngons}
% %\vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccccccc}
% \toprule
% Dataset & \multicolumn{2}{c}{4-gon} & \multicolumn{2}{c}{5-gon} & \multicolumn{2}{c}{6-gon} & \multicolumn{2}{c}{7-gon}\\
% Network & MAE & Time & MAE & Time & MAE & Time & MAE & Time\\
% \midrule
% %Conv1D $G$-avg  & 18.5 $\pm$ 6.8 & 5.9 & 24.1 $\pm$ 4.9 & 11.1 & 23.1 $\pm$ 3.9 & 9.4 & 25.2 $\pm$ 3.3 & 10.1\\ 
% %FC $G$-avg      & 9.4 $\pm$ 0.9 & 2.1 & 13.8 $\pm$ 0.9 & 3.9 & 13.8 $\pm$ 1.0 & 3.1 & 17.2 $\pm$ 1.8 & 3.4\\
% %Message Passing & 259 $\pm$ 65 & 2.0 & 298 $\pm$ 72 & 3.5 & 434 $\pm$ 143 & 2.6 & 457 $\pm$ 156 & 3.0\\
% \textbf{Conv1D $G$-inv (ours)} & \textbf{7.5 $\pm$ 0.5} & 3.0 & \textbf{11.7 $\pm$ 1.8} & 5.5 & \textbf{12.7 $\pm$ 0.6} & 4.5 & \textbf{15.6 $\pm$ 1.3} & 5.4\\ 
% \textbf{FC $G$-inv (ours)} & 8.3 $\pm$ 0.5 & 3.3 & 13.4 $\pm$ 2.1 & 4.1 & 16.6 $\pm$ 1.9 & 4.9 & 22.1 $\pm$ 3.1 & 6.5\\
% %Maron           & 23.4 $\pm$ 1.3 & 10 & 37.2 $\pm$ 4.3 & 13.9 & 48.7 $\pm$ 4.8 & 21.2 & 60.6 $\pm$ 4.0 & 30\\
% %Segment         & 26.8 $\pm$ 2.0 & 1.6& 24.5 $\pm$ 2.1 & 1.8 & 22.9 $\pm$ 1.2 & 2.1 & 24.9 $\pm$ 3.7 & 2.6\\
% %ConvNet & 23.8 $\pm$ 1.8 & 6.3 & 19.8 $\pm$ 1.5 & 6.3 & 24.2 $\pm$ 2.0 & 6.2 & 27.1 $\pm$ 1.3 & 6.3\\  

% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}


% \begin{table}[t]
% \caption{Mean absolute errors [$10^{-3} \text{unit}^2$] and mean running times [ms] in the task of convex n-gon area estimation for several $G$-invariant models. Presented numbers are the mean and standard deviation of MAE for 10 different model instances.}
% \label{tab:ngons}
% %\vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lccc}
% \toprule
% \multicolumn{2}{c}{Dataset} & Conv1D $G$-inv & FC $G$-inv \\
% \midrule
% 4-gon & MAE & 7.5 $\pm$ 0.5 & 8.3 $\pm$ 0.5\\
% & Time & 3.0 & 3.3\\
% 5-gon & MAE & 11.7 $\pm$ 1.8 & 13.4 $\pm$ 2.1\\
% & Time & 5.5 & 4.1\\
% 6-gon & MAE & 12.7 $\pm$ 0.6 & 16.6 $\pm$ 1.9 \\
% & Time & 4.5 & 4.9\\
% 7-gon & MAE & 15.6 $\pm$ 1.3 & 22.1 $\pm$ 3.1\\
% & Time & 5.4 & 6.5 \\

% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}
